Batched Stochastic Bandit for Nondegenerate Functions

This paper studies batched bandit learning problems for nondegenerate functions. We introduce an algorithm that solves the batched bandit problem for nondegenerate functions near-optimally. More specifically, we introduce an algorithm, called Geometric Narrowing (GN), whose regret bound is of order $\widetilde{{\mathcal{O}}} ( A_{+}^d \sqrt{T} )$. In addition, GN only needs $\mathcal{O} (\log \log T)$ batches to achieve this regret. We also provide lower bound analysis for this problem. More specifically, we prove that over some (compact) doubling metric space of doubling dimension $d$: 1. For any policy $\pi$, there exists a problem instance on which $\pi$ admits a regret of order ${\Omega} ( A_-^d \sqrt{T})$; 2. No policy can achieve a regret of order $ A_-^d \sqrt{T} $ over all problem instances, using less than $ \Omega ( \log \log T ) $ rounds of communications. Our lower bound analysis shows that the GN algorithm achieves near optimal regret with minimal number of batches.

==> tex/abs-short.tex <==
This paper studies batched bandit learning problems for nondegenerate functions. Over a compact doubling metric space $(\mathcal{X}, \mathcal{D})$, a function $f : \mathcal{X} \to \mathbb{R}$ is called nondegenerate if there exists $ L \ge \lambda >0 $ and $q \ge 1$, such that 
    $$\lambda ( \mathcal{D} (\mathbf{x}, \mathbf{x}^*) )^q \le f (\mathbf{x}) - f (\mathbf{x}^*) \le L ( \mathcal{D} (\mathbf{x}, \mathbf{x}^*) )^q , \quad \mathbf{x} \in \mathcal{X}, $$
where $\mathbf{x}^* = \arg\min_{\mathbf{z} \in \mathcal{X}} f (\mathbf{z}) $ is the unique minimizer of $f$ over $\mathcal{X}$. In this paper, we introduce an algorithm that solves the batched bandit problem for nondegenerate functions near-optimally. More specifically, we introduce an algorithm, called Geometric Narrowing (GN), whose regret bound is of order $ \widetilde{\mathcal{O}} ( A_+^d \sqrt{T} ) $, where $d$ is the doubling dimension of $(\mathcal{X},\mathcal{D})$, and $A_+$ is a constant independent of $ d $ and the time horizon $T$. In addition, GN only needs $ {\mathcal{O}} (\log \log T) $ batches to achieve this regret. We also provide lower bound analysis for this problem. More specifically, we prove that over some (compact) doubling metric space of doubling dimension $d$: 1. For any policy $\pi$, there exists a problem instance on which $\pi$ admits a regret of order ${\Omega} ( A_-^d \sqrt{T} )$, where $A_-$ is a constant independent of $ d $ and $T$; 2. No policy can achieve a regret of order $ A_-^d \sqrt{T} $ over all problem instances, using less than $ \Omega ( \log \log T ) $ rounds of communications. Our lower bound analysis shows that the GN algorithm achieves near optimal regret with minimal number of batches. 

==> tex/acknowledgement.tex <==
\section*{Acknowledgement}

T. Wang is partially supported by the Shanghai Sailing Program (No. 24YF2702500) and a grant from DeepVerse Inc. 
T. Wang also thanks Shanghai Institute for Mathematics and
Interdisciplinary Sciences (SIMIS) for their financial support. This research was partially funded by SIMIS under grant number SIMIS-ID-2024-CN and SIMISID-2024-WE. T. Wang is grateful for the resources and facilities provided by SIMIS, which were essential for the completion of this work.
